Fuzzy PSI from Symmetric Primitives with Exact Logarithmic Dependence on Distance Threshold

Previous FPSI works have demonstrated a linear scaling with the distance threshold $\delta$, while some recent works have achieved a poly-logarithmic dependence on $\delta$. However, these protocols either support only the $L_\infty$ distance, or they support general $L_{p\in[1,\infty]}$ distances but rely on expensive additive homomorphic encryption (AHE). Achieving exact logarithmic dependence on $\delta$ for general $L_{p\in[1,\infty]}$ distances without relying on costly AHE would constitute a theoretical breakthrough in optimal threshold scaling and a practical advance toward scalable FPSI applications. In this work, we present new FPSI protocols for $L_{p\in[1,\infty]}$ distances that are entirely built from oblivious transfer (OT) and symmetric-key primitives. We propose FPSI protocols based on both the apart and the separate assumptions, which are applicable to low- and high-dimensional settings, respectively. Our constructions achieve strictly logarithmic complexity in $\delta$, which is optimal in the sense that distinguishing all values in an interval of length $O(\delta)$ necessarily requires $\Omega(\log \delta)$ bits of information. Our core idea is to perform fuzzy matching via prefix representation and interactively determine the correct prefix using equality conditions. To this end, we propose a suite of new components that can be implemented efficiently using only OT and symmetric-key operations. We implement our FPSI protocols and compare them with the state-of-the-art FPSI protocols for $L_{p\in[1,\infty]}$ distance. Experiments show that our protocols outperform the prior state-of-the-art by up to $43.7\times$ in runtime and $31.3\times$ in communication.

==> 7-Conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this work, we propose new FPSI protocols for $L_{p\in[1,\infty]}$ distance. Our construction primarily relies on OT and symmetric-key cryptographic primitives, achieving significant efficiency gains — up to $142.1\times$ faster runtime and $13.8\times$ lower communication overhead compared to prior schemes. 
%Although our protocol relies on a slightly stronger assumption than previous protocols, similar to previous work, we have demonstrated that when the input is randomly selected, there is an overwhelming probability that this assumption holds. A highly valuable future work would be to weaken assumptions while maintaining high efficiency. Another possible direction is to enhance the protocol to malicious security.
While our protocol requires a slightly stronger assumption than previous work, we rigorously prove that this assumption holds with overwhelming probability when inputs are randomly sampled. 
A promising direction for future research is to relax this assumption while retaining high efficiency. Additionally, extending the protocol to achieve malicious security is another promising direction.
